A Planning Framework for Adaptive Labeling

Ground truth labels/outcomes are critical for advancing scientific and engineering applications, e.g., evaluating the treatment effect of an intervention or performance of a predictive model. Since randomly sampling inputs for labeling can be prohibitively expensive, we introduce an adaptive labeling framework where measurement effort can be reallocated in batches. We formulate this problem as a Markov decision process where posterior beliefs evolve over time as batches of labels are collected (state transition), and batches (actions) are chosen to minimize uncertainty at the end of data collection. We design a computational framework that is agnostic to different uncertainty quantification approaches including those based on deep learning, and allows a diverse array of policy gradient approaches by relying on continuous policy parameterizations. On real and synthetic datasets, we demonstrate even a one-step lookahead policy can substantially outperform common adaptive labeling heuristics, highlighting the virtue of planning. On the methodological side, we note that standard REINFORCE-style policy gradient estimators can suffer high variance since they rely only on zeroth order information. We propose a direct backpropagation-based approach, Smoothed-Autodiff, based on a carefully smoothed version of the original non-differentiable MDP. Our method enjoys low variance at the price of introducing bias, and we theoretically and empirically show that this trade-off can be favorable.

==> UQ/abstract.tex <==
Since ML models are always in operation, they often encounter inputs unseen during training. Uncertainty quantification (UQ) methods aim to capture when models are unreliably extrapolating, a foundational goal in trustworthy AI, active learning, and exploration in reinforcement learning. These downstream goals necessitate  i) reliable UQ performance on out-of-distribution (OOD) inputs, and ii) the ability to reliably sharpen beliefs as more data is gathered (which we term “posterior consistency”). We present \textsf{UQBench}, a comprehensive benchmarking framework that can evaluate UQ algorithms over distribution shifts and posterior consistency, and instantiate it on several real-world datasets. Our benchmark highlights several methodological challenges that are unobservable on existing UQ benchmarks that solely focus on static in-distribution (ID) settings. Due to tremendous variation in UQ quality across hyperparameters, we observe a direct tension between ID and OOD performance. These challenges magnify in the dynamic setting where posteriors are updated based on new observations. Our benchmark underscores the need for reliable posterior update methods, an often overlooked dimension in UQ algorithmic development focusing on static performance. 

% Uncertainty quantification (UQ) is important for many downstream tasks beyond supervised learning, such as active learning, and exploration in reinforcement learning. To achieve desired performance, UQ methodologies need to enable reliable priors, characterize uncertainty in  out-of-support data and update consistently  as new data is observed. We show existing UQ benchmarks fail to fairly evaluate the UQ methodologies on these aspects, which we call “posterior consistency”. To reliably estimate and benchmark different UQ methodologies on these dimensions, we propose an open-source benchmark that introduces datasets, commonly occurring practical out-of-distribution settings, and evaluates state-of-the-art UQ modules using standard metrics such as joint log-loss and marginal log-loss. In addition, we operationalize the evaluation of  “posterior consistency” for modern deep learning-based UQ methods, to measure  the noise in a UQ update, by tying it to canonical training practices of these methods such as different training seeds and early stopping. We demonstrate that the current methodologies such as Ensembles, ENNs, are unable to reliably encode prior information, require extensive hyperparameter tuning and ad-hoc mechanisms to achieve reliable performance. The proposed benchmark serves as a comprehensive evaluation of UQ modules to enable complex downstream tasks. 

==> UQ/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
   \answerYes{} See Section~\ref{sec:introduction} and Section~\ref{sec:conclusion}.
  \item Did you describe the limitations of your work?
      \answerYes{}   See Section~\ref{sec:introduction} and Section~\ref{sec:conclusion}.
  \item Did you discuss any potential negative societal impacts of your work?
     \answerYes{}   See Section~\ref{sec:introduction} and Section~\ref{sec:conclusion}.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
      \answerYes{} 
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? We provide these in the supplemental material.
    \answerYes{}{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?  
      \answerYes{}
See Section~\ref{sec:details-experiments} and Section~\ref{sec:experiments-other-datasets}.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}  See Section~\ref{sec:details-experiments}.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} See Section~\ref{sec:benchmark}.
  \item Did you mention the license of the assets?
    \answerYes{} See Section~\ref{sec:benchmark}.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} See the supplemental material.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix

% \section{Appendix}

% Include extra information in the appendix. This section will often be part of the supplemental material. Please see the call on the NeurIPS website for links to additional guides on dataset publication.

% \begin{enumerate}

% \item Submission introducing new datasets must include the following in the supplementary materials:
% \begin{enumerate}
%   \item Dataset documentation and intended uses. Recommended documentation frameworks include datasheets for datasets, dataset nutrition labels, data statements for NLP, and accountability frameworks.
%   \item URL to website/platform where the dataset/benchmark can be viewed and downloaded by the reviewers.
%   \item URL to Croissant metadata record documenting the dataset/benchmark available for viewing and downloading by the reviewers. You can create your Croissant metadata using e.g. the Python library available here: https://github.com/mlcommons/croissant
%   \item Author statement that they bear all responsibility in case of violation of rights, etc., and confirmation of the data license.
%   \item Hosting, licensing, and maintenance plan. The choice of hosting platform is yours, as long as you ensure access to the data (possibly through a curated interface) and will provide the necessary maintenance.
% \end{enumerate}

% \item To ensure accessibility, the supplementary materials for datasets must include the following:
% \begin{enumerate}
%   \item Links to access the dataset and its metadata. This can be hidden upon submission if the dataset is not yet publicly available but must be added in the camera-ready version. In select cases, e.g when the data can only be released at a later date, this can be added afterward. Simulation environments should link to (open source) code repositories.
%   \item The dataset itself should ideally use an open and widely used data format. Provide a detailed explanation on how the dataset can be read. For simulation environments, use existing frameworks or explain how they can be used.
%   \item Long-term preservation: It must be clear that the dataset will be available for a long time, either by uploading to a data repository or by explaining how the authors themselves will ensure this.
%   \item Explicit license: Authors must choose a license, ideally a CC license for datasets, or an open source license for code (e.g. RL environments).
%   \item Add structured metadata to a dataset's meta-data page using Web standards (like schema.org and DCAT): This allows it to be discovered and organized by anyone. If you use an existing data repository, this is often done automatically.
%   \item Highly recommended: a persistent dereferenceable identifier (e.g. a DOI minted by a data repository or a prefix on identifiers.org) for datasets, or a code repository (e.g. GitHub, GitLab,...) for code. If this is not possible or useful, please explain why.
% \end{enumerate}

% \item For benchmarks, the supplementary materials must ensure that all results are easily reproducible. Where possible, use a reproducibility framework such as the ML reproducibility checklist, or otherwise guarantee that all results can be easily reproduced, i.e. all necessary datasets, code, and evaluation procedures must be accessible and documented.

% \item For papers introducing best practices in creating or curating datasets and benchmarks, the above supplementary materials are not required.
% \end{enumerate}

==> details_UQ.tex <==
\section{Details of benchmarking UQ modules} \label{sec:details-benchmark-UQ}







\subsection{Notation summary}
\begin{itemize}
    \item $T$ horizons
    \item $x \sim p_x$, $p(Y|X,f\sim\mu) = \int \prod_{i} p(y_i|f,{\mathbf x_i}) d\mu(f)$
    \item Initial training data - $(X^0,Y^0) =({\mathbf x}_{1:m}^0,y_{1:m}^0)$
    \item Queried unlabeled data set in step $j$ - $X^j$ , corresponding queried labels  are $Y^j$. 

    \item $f \sim \pi$. Further, posteriors are defined as follows:
\begin{itemize}
    \item  $\mu_0$ informed by $[\mu, (X^0,Y^0)]$ 
    \item  $\mu_j$ informed by $[\mu_{j-1}, (X^j,Y^j) ]$ or $[\mu, \cup_{i=0}^{j}(X^i,Y^i)]$
\end{itemize}
   

    \item Unlabelled set - $X^u = ({\mathbf x}_{1:n}^{u}) $.
    \item Pool set at step $j$ - $X^{pool, j}$
    
\end{itemize}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

